Representation Learning on Graphs: Methods and Applications

Machine learning on graphs is an important and ubiquitous task with applications ranging from drug design to friendship recommendation in social networks. The primary challenge in this domain is finding a way to represent, or encode, graph structure so that it can be easily exploited by machine learning models. Traditionally, machine learning approaches relied on user-defined heuristics to extract features encoding structural information about a graph (e.g., degree statistics or kernel functions). However, recent years have seen a surge in approaches that automatically learn to encode graph structure into low-dimensional embeddings, using techniques based on deep learning and nonlinear dimensionality reduction. Here we provide a conceptual review of key advancements in this area of representation learning on graphs, including matrix factorization-based methods, random-walk based algorithms, and graph neural networks. We review methods to embed individual nodes as well as approaches to embed entire (sub)graphs. In doing so, we develop a unified framework to describe these recent approaches, and we highlight a number of important applications and directions for future work.

==> Makefile <==
RCSFLAGS= -l
MAIN=paper-repgraph
TEXPARTS= \
#	000abstract.tex		\
	010intro.tex		\
	020related.tex		\
	030proposed.tex	\
	040experiments.tex	\
	050discussion.tex	\
	060conclusion.tex	\
	070appendix.tex

BIBPARTS= *.bib
LPR = pspr # or change to 'qpr -q ps3'
POSTSCRIPT= dvips -P cmz -t letter  #dvips -f
FIGPARTS = FIG

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

try: $(MAIN).tex
	pdflatex $(MAIN)

print: $(MAIN).ps
	$(LPR) $(MAIN).ps

clean:
	\rm -f *.dvi $(MAIN).pdf *.bbl *.aux *.blg *.fdb_latexmk *.fls *.synctex.gz *.log *.blg *.toc all.tar* uu *~ *.bak

spotless: clean
	\rm -f $(MAIN).pdf

all.tar:
	tar cvfh all.tar makefile $(MAIN).tex $(TEXPARTS) $(BIBPARTS) \
	$(FIGPARTS) README

uu: all.tar
	gzip all.tar
	uuencode all.tar.gz all.tar.gz > uu

bundle.all: $(TEXPARTS) 
	bundle  README $(TEXPARTS) $(BIBPARTS) makefile > bundle.all

zip:
	cmd /C "pkzip $(MAIN).zip -P $(MAIN).pdf Makefile *.cls *.tex *.bib FIG/*.eps"

